Explicit shading strategies for repeated truthful auctions

With the increasing use of auctions in online advertising, there has been a large effort to study seller revenue maximization, following Myerson's seminal work, both theoretically and practically. We take the point of view of the buyer in classical auctions and ask the question of whether she has an incentive to shade her bid even in auctions that are reputed to be truthful, when aware of the revenue optimization mechanism. We show that in auctions such as the Myerson auction or a VCG with reserve price set as the monopoly price, the buyer who is aware of this information has indeed an incentive to shade. Intuitively, by selecting the revenue maximizing auction, the seller introduces a dependency on the buyers' distributions in the choice of the auction. We study in depth the case of the Myerson auction and show that a symmetric equilibrium exists in which buyers shade non-linearly what would be their first price bid. They then end up with an expected payoff that is equal to what they would get in a first price auction with no reserve price. We conclude that a return to simple first price auctions with no reserve price or at least non-dynamic anonymous ones is desirable from the point of view of both buyers, sellers and increasing transparency.

==> GenParetoComps.tex <==
\subsection{Problem setup}
\newcommand{\GP}{\text{GP}}

We suppose that bidder $1$ has value $X_1$ for the item. The distribution of $X_1$ is generalized pareto. We assume that she is strategic and will send the seller another generalized Pareto distribution, say $X_2$ as her value. As we show below, this amounts to a non-linear shading. 

We assume that the seller knows that the distribution of the bidders is Generalized Pareto, the seller runs a Myerson auction and the other bidders are non-strategic. 

\subsubsection{Reminders}
If $X$ is Generalized Pareto (GP) with parameters $(\sigma,\xi)$, we have, when $\xi<0$, 
$$
P(X\geq t)=(1+\xi t/\sigma)^{-1/\xi}\;.
$$
and otherwise $P(X\geq t)=\exp(-t/\sigma)$ if $\xi=0$. The support is $[0,-\sigma/\xi]$. 

We note that 
\begin{itemize}
\item $$\Exp{X}=\frac{\sigma}{1-\xi}\;.$$
\item The virtual value is 
$$
\phi(x)=(1-\xi)\left(x-\Exp{X}\right)\;.
$$
\item In particular, the optimal reserve price, $r^*$ is such that 
$$
r^*=\Exp{X}\;.
$$
\item We have the stochastic representation 
$$
X=\frac{\sigma}{\xi}(U^{-\xi}-1)\;, \text{ where } U\sim \text{Unif}[0,1]\;.
$$
\end{itemize}
\textcolor{red}{Note: we could add a mean shift}
In particular, if $X_1\sim \GP(\sigma_1,\xi_1)$, 
$$
X_t=\frac{\sigma_t}{\xi_t} \left(\left[1+\frac{\xi_1}{\sigma_1}X_1\right]^{\frac{\xi_t}{\xi_1}}-1\right)\sim \GP(\sigma_t,\xi_t)\;.
$$
This is of course a non-linear shading. 
\textcolor{red}{totally secondary self-note: it's of course very easy to generate a random variable Y with cdf $F_Y$ as a function of another one, $X$: essentially $Y=F_Y^{-1}F_X(X)$ has the right distribution, since $F_X(X)$ is uniform on $[0,1]$. The computations below assume that $X_t$ is a deterministic function of $X_1$. However, one could do a stochastic/random shading. The idea here would be to use copulas to get another bivariate distribution whose marginal are $X_1$ and $X_t$ but whose joint is different from the one implied above. It's highly unlikely this (i.e. optimizing the copula) would help, but if using deterministic shadings was a problem, one could come up rather easily with stochastic ones.}
\subsubsection{Technical problem setup}
Suppose bidder 1, whose value for the item is $X_1$ bids according to $X_t\sim GP(\sigma_t,\xi_t)$. As we showed above, incentive compatibility is lost in GP auctions, so our question makes (some) sense.

We assume that the other bidders are non-strategic; we call $Y_i$ their values, assume that their distributions are regular and call $V_i=\phi_i(Y_i)$, where $\phi_i$ is the virtual value associated with the distribution of $Y_i$. \textcolor{red}{cumbersome English... } Finally, we call 
$$
Z\triangleq \max(0,V_i)\;.
$$
$Z$ is the competition bidder 1 faces in terms of virtual valuation. 

Recall that that the expected payment of bidder 1 when he bids using $X_t$ is 
$$
\Exp{\phi_t(X_t)1_{\phi_t(X_t)\geq Z}}\;.
$$
(see \cite{krishna2009auction}, p. 67 and \cite{RoughgardenTLA2016} \textcolor{red}{i should recheck, give precise ref}) 
We have for the expected payoff
$$
\Pi(t)=\Exp{(X_1-\phi_t(X_t))1_{\phi_t(X_t)\geq Z}}\;.
$$
Assuming independence of $Z$ and $X_1$ and hence $X_t$, we have by conditioning on $X_1$, calling $F_Z$ the cdf of $Z$, 
$$
\Pi(t)=\Exp{(X_1-\phi_t(X_t))F_Z(\phi_t(X_t))}\;.
$$
Using the stochastic representation discussed above, we see that 
\begin{align*}
\phi_t(X_t)&=(1-\xi_t)\sigma_t \left[\frac{U^{-\xi_t}-1}{\xi_t}-\frac{1}{1-\xi_t}\right]\;,\\
X_1&=\frac{\sigma_1}{\xi_1}(U^{-\xi_1}-1)\;.
\end{align*}
$\Pi(t)$ is therefore a simple function of the parameters of interest. Note that the dependence of $\phi_t(X_t)$ on $\sigma_t$ is linear. In particular, 
$$
\frac{\partial \phi_t(X_t)}{\partial \sigma_t}=\frac{\phi_t(X_t)}{\sigma_t}=\frac{1-\xi_t}{\sigma_t}X_t-1\;.
$$
On the other hand, 
$$
\frac{1}{\sigma_t}\frac{\partial \phi_t(X_t)}{\partial \xi_t}=-\frac{1}{\xi^2}(U^{-\xi}-1)-\ln(U)U^{-\xi}(\frac{1}{\xi}-1))\;.
$$
In other words, 
$$
\frac{\partial \phi_t(X_t)}{\partial \xi_t}=-\frac{1}{\xi_t}X_t+\frac{1-\xi_t}{\xi_t}\left(X_t+\frac{\sigma_t}{\xi_t}\right)\ln(1+\frac{\xi_t}{\sigma_t}X_t)
$$
Another random thing: suppose that $X_\mu=\mu+X$. Then it is easy to verify that $\phi_\mu(x)=\mu+\phi(x-\mu)$. In particular, $\phi_\mu(X_\mu)=\mu+\phi(X)$. 

\paragraph{Back to general case}Of course $F_Z(x)=\prod_{i=1}^K F_{V_i}(x)1_{x\geq 0}$, so $F_Z$ is discontinuous at zero. Of course we can still differentiate it in the sense of distributions, though a point mass at 0 appears. So its differential in the sense of distributions is just $\prod_{i=1}^K F_{V_i}(0) \delta_0$ at 0. Below we ignore that and when we can justify a posteriori that it's OK.

So we find that, with $f_Z$ denoting the derivative of $F_Z$ that formally and (ignoring the point mass issue)
$$
\frac{\partial}{\partial t} \Pi(t)=\Exp{\frac{\partial}{\partial t} \phi_t(X_t) [(X_1-\phi_t(X_t))f_Z(\phi_t(X_t))-F_Z(\phi_t(X_t))]}\;.
$$
Note that $f_Z(x)=F_Z(x)=0$ when $x\leq 0$ with our slight abuse of notation. 

\textcolor{blue}{Above is basically designed to guess a solution if everything goes well. If we include the point mass problem we should get
\begin{align*}
\frac{\partial}{\partial t} \Pi(t)&=\Exp{\frac{\partial}{\partial t} \phi_t(X_t) [(X_1-\phi_t(X_t))f_Z(\phi_t(X_t))-F_Z(\phi_t(X_t))]}
\\
&\textcolor{red}{+\left.\frac{\partial}{\partial t}\phi_t(X_t)\right|_{\phi_t(X_t)=0}\prod_{i=1}^K F_{V_i}(0) f_{X_1}(x_1) x_1}\;,
\end{align*}
where $x_1$ is such that $x_t=g(x_1)$ and $\phi_t(x_t)=0$. 
Note that if a solution is such that $V_i$ are supported on $\mathbb{R}_+$ or $x_1=0$ whenever $\phi_t(x_t)=0$ and $x_t=g(x_1)$, then we can rigorously ignore this extra term.
As we will see in the symmetric equilibrium case, that is indeed the case...}


\paragraph{``Practical" aspects} Suppose we happen to know $F_Z$. Then we can compute the gradient of $\Pi(t)$ at any time $t$. Note also that the expectation in question can be computed by integrating a function of a uniform random variable. 

In case interpretation is in doubt think of above expression as a directional derivative; of course it's in probability measure space but as explain above we could view of all this as e.g a perturbation in hazard rate space and have no problem. Can think of $t$ as a scalar parameter if the direction of perturbation is given. Basically here we do not make explicit the $\frac{\partial}{\partial t} \phi_t(X_t)$ but it all makes sense. 
\subsection{Random self comments}
Considering $(X_1-\phi_t(X_t))f_Z(\phi_t(X_t)-F_Z(\phi_t(X_t)$ and trying to optimize $\Pi(t)$ it's natural to ask how we can leverage the equation 
\begin{equation}\label{eq:naiveStabilityEquation}
(X_1-\phi_t(X_t))f_Z(\phi_t(X_t)-F_Z(\phi_t(X_t))=0\;, \text{ when } \phi_t(X_t)\geq 0\;.\tag{naive-stab-equation}
\end{equation}
Of course, we can rewrite that as 
$$
X_1=\phi_t(X_t)+\frac{F_Z(\phi_t(X_t))}{f_Z(\phi_t(X_t))}\;.
$$
Below I call $W_t=\phi_t(X_t)$. Some simple observations
\begin{enumerate}
\item Given $Z_t$ it's of course trivial to find an $X_1$ for which Equation \eqref{eq:naiveStabilityEquation} is satisfied. Depending on $Z$, even if $X_t$ is generalized Pareto, $X_1$ may not be GP. Though of course, it gives us a mapping...
\item Multiplayer equilibrium probably solvable in the same way with $Z$ being equal in law to $\max(0,\{Z_t^{(i)}\}_{i=2}^K)$, $K$ being total number of players; and us being player 1. 
\item Otherwise, we get the representation 
$$
W_t=(\id+F_Z/f_Z)^{-1}(X_1)\;.
$$
One question is whether that is a r.v corresponding to a virtual value; note that we only need this representation when $W_t>0$, so that may help. (In particular, $\Exp{W_t}=0$ unless we are in a pathological situation.) Note that we need to send $X_t$ and not $W_t$. So the question is really whether we can learn $\phi$ from $W$. So we suppose we can sample from $\phi_X(X)$ without knowing $X$. Note that $P(\phi_X(X)\leq t)=F_X(\phi^{-1}(t))$. Also, \textcolor{red}{need to recheck that}$\Exp{\phi_X(X)1_{\phi_X(X)\leq t}}=\phi_X^{-1}(t)[F_X(\phi^{-1}(t))-1]$. So it seems that 
$$
\phi^{-1}(t)=\frac{\Exp{\phi_X(X)1_{\phi_X(X)\leq t}}}{P(\phi_X(X)\leq t)-1}=\frac{\Exp{W1_{W\leq t}}}{P(W\leq t)-1}\;.
$$
So assuming the above is correct, we can compute invert the relation between $X$ and $W$. 
\item Seems that if competition is generalized pareto computing $F/f$ (corresponding to competition virtual values) is very easy. In particular, $\phi_t(X_t)$ linear in $X_1$ for $\phi_t(X_t)>0$. On the other side of 0, maybe can fit another linear function of $X_1$ so that we get $\phi_t(X_t)$ to be continuous as function of $X_1$ and have mean 0. Of course should be possible to get non discontinuity in derivative. 
\end{enumerate}

\subsection{Computation of $F_\phi$ and $f_\phi$ in GP families}
\begin{lemma}
Suppose $W$ has a Generalized Pareto distribution. Call $F_W$ the cdf of $W$ and $f_W$ its density. 

If $Z=\phi_W(W)$, where $\phi_W$ is the virtual value of $W$, we have
$$
\frac{F_Z(t)}{f_Z(t)}=c_\phi \frac{F_W(\phi^{-1}(t))}{f_W(\phi^{-1}(t))}\;,
$$
where $c_\phi=\phi_W'(t)$. If $r^*$ is the monopoly price associated with $W$, we more specifically have 
$$
\frac{F_Z(t)}{f_Z(t)}=c_\phi \frac{F_W(t/c_\phi+r^*)}{f_W(t/c_\phi+r^*)}\;.
$$
\end{lemma}

\begin{proof}
Note that the $F_Z$ that appears above is really the cdf of $\phi(W)$, where $\phi$ is the virtual value of $W$. Hence, 
$$
F_Z(t)=P(Z\leq t)=P(\phi(W)\leq t)=F_W(\phi^{-1}(t))\;.
$$
In particular, 
$$
f_Z(t)=\frac{f_W(\phi^{-1}(t))}{\phi'(\phi^{-1}(t))}\;.
$$
In Generalized Pareto families, $\phi$ is linear, so that $\phi'$ is a constant, because $\phi(t)=c_\phi(t-r^*)$, where $r^*$ is the monopoly price. The first result follows immediately. Noticing that $\phi^{-1}(x)=x/c_\phi+r^*$ gives the second result.  
\end{proof}
\subsection{How to shade for boosted second price auctions/Myerson with only GPs}
Suppose that buyer 1 has value distribution $F_1$ and associated random variable $X_1$. Facing boosted second price auctions, she might want to shade in such a way that her bids have a generalized Pareto distribution so she is effectively facing a Myerson auction. So if 
$$
\mathfrak{p}=(\sigma,\xi)\;,
$$ 
her payoff is 
$$
\Pi(\mathfrak{p})=\Exp{(X_1-\phi_\mathfrak{p}(X_\mathfrak{p}))F_Z(\phi_\mathfrak{p}(X_\mathfrak{p}))}
$$
and she seeks to find 
$$
\mathfrak{p}^*=\argmax_{\mathfrak{p}}\Pi(\mathfrak{p})\;.
$$
Note that under mild regularity conditions $U_1=F_1(X_1)$ has uniform distribution. So it is natural for her to send the bid 
$$
X_\mathfrak{p}=\frac{\sigma}{\xi}\left[(1-F_1(X_1))^{-\xi}-1\right]\;,
$$
which will have a GP($\mathfrak{p}$) distribution. Furthermore, the bid sent is then increasing with $X_1$ (if we had used $[F_1(x_1)]^{-\xi}$ it would have been decreasing with $x_1$). Hence the problem she faces is a two dimensional optimization problem. 

\subsubsection{Uniform adversaries} 
Suppose she faces $K$ adversaries who send independent bids that are distributed according to a Uniform[0,1] distribution. Elementary computations show that 
$$
F_Z(t)=[(t+1)/2]^K 1_{t\geq 0}\;.
$$
So the problem becomes 
$$
\max_{\mathfrak{p}}\Exp{[X_1-\phi_{\mathfrak{p}}(X_\mathfrak{p})][(\phi_{\mathfrak{p}}(X_\mathfrak{p})+1)/2]^K 1_{\phi_{\mathfrak{p}}(X_\mathfrak{p})\geq 0}}\;.
$$
Now recall that 
$$
\nabla_{\mathfrak{p}}\phi_\mathfrak{p}(X_\mathfrak{p})=\begin{bmatrix}
\frac{\phi_\mathfrak{p}(X_\mathfrak{p})}{\sigma}=\frac{(1-\xi)X_\mathfrak{p}-\sigma}{\sigma}\\
-\frac{1}{\xi}X_\mathfrak{p}+\frac{1-\xi}{\xi}(X_\mathfrak{p}+\frac{\sigma}{\xi})\ln(1+\frac{\xi}{\sigma}X_\mathfrak{p})
\end{bmatrix}
$$
\newcommand{\phiAtShaded}{\phi_\mathfrak{p}(X_\mathfrak{p})}
So for the payoff $\Pi(\mathfrak{p})$, we have 
\begin{align*}
2^K\nabla \Pi(\mathfrak{p})&=\Exp{\nabla_{\mathfrak{p}}[\phiAtShaded][\phiAtShaded+1]^{K-1}[KX_1-(K+1)\phiAtShaded-1]1_{\phiAtShaded\geq 0}}\\
&+\begin{bmatrix}
0\\
-\frac{1}{\xi(1-\xi)}-\frac{1}{\xi^2}\ln(1-\xi) 
\end{bmatrix}
\gamma_1(\xi)
\end{align*}
where 
$$
\gamma_1(\xi)=F_1^{-1}((1-\xi)^{1/\xi})f_1(F_1^{-1}((1-\xi)^{1/\xi}))
$$
Note that when $\phiAtShaded=0$, the corresponding $U$ is equal to $(1-\xi)^{1/\xi}$. \textcolor{red}{need to recheck this as it may have come from an erroneous setup}

We note that this gradient is a relatively explicit function of $(\sigma,\xi)$ and hence we can seek to numerically find its roots and local extrema of $\Pi$. 

In certain limited situations, we can also find explicit 
solutions. 

\begin{lemma}
Suppose that $X_1$ is GP($\sigma_1,\xi_1$) with $\frac{\sigma_1}{1-\xi_1}=\frac{1}{K}$. Suppose further that 
$$
-\frac{1-\xi_1}{\xi_1}\ln(1-\xi_1)=1\;.
$$
Then taking 
$$
x_t=\frac{K}{K+1}\frac{x_1}{1-\xi_1}\;,
$$
we have $X_t$ is GP($\sigma_1\frac{K}{(K+1)(1-\xi_1)},\xi_1$). 
Furthermore, the corresponding $\Pi(\mathfrak{p})$ has gradient 0 at this $\mathfrak{p}$. 
\end{lemma}

\begin{proof}
Use all the results below, noticing that for this $\xi_1$, which is non-positive, the ``extra term'' in the gradient coming from the point mass issue is 0. 
Then we can re-use all the work below, because we just have to solve $\phi_t(X_t)=(X_1-1/K)/(1+1/K)$. 
If I wanted to get rid of the condition $\sigma_1/(1-\xi_1)=1/K$, I would have to allow $X_t$ to be a GP with mean shift. A priori that may change the form of $\phi$... so that would lead to a slightly different problem.
\end{proof}

\subsubsection{Numerics}
We start with the case where $X_1\sim Unif[0,1]$, $X_1$ is strategic but her adversaries are not. Then $X_\mathfrak{p}=\frac{\sigma}{\xi}((1-X_1)^{-\xi}-1)$. Then $\gamma_1(\xi)=(1-\xi)^{1/\xi}$. 

\paragraph{3 players; 1 strategic} In this case, we implement the shading we just discussed, though it may not be optimal. 
When being truthful, we have a payoff of roughly 0.08325.
\begin{verbatim}
K=2.0
sigma_K = 1/(K+1.0)
xi=-1.0
sigma = 1.0
temp = computePayoff(x1000,sigma,xi,unifQuantileFunction,
cdf_vvalue_unif,number_opponents=K)
print(temp)
0.08325
\end{verbatim}
Whereas when we shade according to what is explained above, we get an expected payoff of roughly 0.139, almost 50\% higher. More precisely, we use for the shading $\sigma^{(2)}=1/3$ and $\xi=-1$ since we start from $X_1$ being uniform, so $\sigma=1$ and $\xi_1=-1$. 
\begin{verbatim}
temp2 = computePayoff(x1000,sigma_K,xi,unifQuantileFunction,
cdf_vvalue_unif,number_opponents=K)
print(temp2)
0.138916666667
\end{verbatim}


\subsection{An example: uniform adversaries}
\textcolor{red}{The case $K=1$ is problematic for below when $X$ is itself uniform[0,1]. Need to clarify... Stems probably from the fact that cannot ignore the extra term in my derivation of the expected profit...  }
We suppose here that $W$ is uniform [0,1]. In this case, $F_W/f_W=\id$, so that 
$$
\frac{F_Z}{f_Z}(t)=t+c_\phi r^*;.
$$
Note that for Generalized Paretos, we have $r^*=\frac{\sigma}{1-\xi}$ and $c_\phi=(1-\xi)$, so that $c_\phi r^*=\sigma$. 

If one player is facing $K$ adversaries with values that are uniform[0,1], we see that for $t>0$, 
$$
\frac{F^{\otimes_{K}}_Z}{f^{\otimes_{K}}_Z}(t)=\frac{1}{K}\frac{F_Z}{f_Z}(t)\;.
$$
So we conclude that the equation characterizing $\phi_t(X_t)$ is just, when $\phi_t(X_t)>0$,
$$
\left(1+\frac{1}{K}\right) \phi_t(X_t)+\frac{1}{K}=X_1\;.
$$
In other words, 
$$
\phi_t(X_t)=\frac{X_1-\frac{1}{K}}{1+\frac{1}{K}}, \; \; X_1\geq \frac{1}{K}\;.
$$
\textcolor{red}{Note: if $X_1$ is uniform [0,1] we have a problem b/c $X_1\leq 1/K$ if $K=1$. So $\phi_t(X_t)$ as defined above cannot be positive; so need to review setup in this case; or no shading really possible or necessary? direct computation reveals same behavior. the derivative computed above is always negative; more work needed on directional derivative of $\phi_t(X_t)$. note that symmetric case avoids all these problems. Explanations above most likely...}

As explained below, if we take $X_t=g(X_1)$ with 
$$
g(x)=\frac{K}{K+1}\frac{\int_x^{\infty} (u-1/K) f_1(u) du}{1-F_1(x)}\;,
$$
we will have 
$$
\phi_t(x_t)=\frac{x_1-1/K}{1+1/K}\;.
$$
More explicitly, if $X_1$ is $GP(\sigma_1,\xi_1)$, using Equation \eqref{eq:meanGPs} on page \pageref{eq:meanGPs}, we have 
$$
\boxed{
g(x)=\frac{K}{K+1}\left[\frac{x}{1-\xi_1}+\left(\frac{\sigma_1}{1-\xi_1}-\frac{1}{K}\right)\right]
}
$$
As noted after the derivation of Equation \eqref{eq:meanGPs}, we have $(x+\sigma_1)/(1-\xi_1)\geq x$, so that $g(x)\geq 0$ whenever $x\geq 1/K$. In other words, $\phi_t(X_t)\geq 0$ whenever $X_1\geq 1/K$. 

We note that if $Y$ is GP($\sigma,\xi$), $\alpha Y$ is GP($\sigma \alpha,\xi$). So $g(X_1)$ is a shifted version of the family of GPs we consider here; in case $\Exp{X_1}=\frac{\sigma_1}{1-\xi_1}-1/K$, we have member of the GP family we considered here. See also comps below which were done before and are less general. Otherwise we get a shifted version; in the generalization of GPs families to a location-scale family, that is fine. 

\paragraph{Important side note concerning sending a negative bid! (And why we don't need to do it)} Note that if we want our pseudo-bids to be positive, we either have a constraint on $\sigma_1,\xi_1$ and $K$ or we need to take our bid $\max(g(x),0)$. Of course that has little impact on the whole story, since if $\Gamma$ is a random variable and $\Gamma_{x_0}=\max(\Gamma,x_0)$, i.e. a truncation of $\Gamma$ at $x_0$, we have with obvious notations 
$\phi_{\Gamma_{x_0}}(t)=\phi_{\Gamma}(t)$ if $t>x_0$ and $\phi_{\Gamma_{x_0}}(t)=-\infty$ if $t<x_0$. At $t=x_0$, things are bit ambiguous, but $\phi_{\Gamma_{x_0}}$ can probably be taken to be $\phi_{\Gamma}(x_0)$; there is no density so we have to either define it as a right derivative or fix it somehow. Conclusion of this interlude is that no matter what, if we take $\tilde{x}_t=\max(g(x_1),0)$, we have for $x_1\geq 1/K$ $\phi(\tilde{x}_t)=\frac{x_1-1/K}{1+1/K}$ for $x_1\geq 1/K$. 
% If $\Exp{X_1}\neq \frac{1}{K}$, this shading cannot be used  everywhere, since for nice distributions, $\Exp{\phi_t(X_t)}=0$.  
% But it is natural to find another linear shading on the other side of $\frac{1}{K}$, i.e.
% $$
% \phi_t^{-}(X_t)=a^{-}(X_1-\frac{1}{K})\;.
% $$
% The condition $\Exp{\phi_t^{-}(X_t)}=0$ gives as candidate
% $$
% a^{-}=\frac{1}{1+1/K}\frac{\Exp{[X_1-\frac{1}{K}]1_{[X_1-\frac{1}{K}]\geq 0}}}{\Exp{[-X_1+\frac{1}{K}]1_{[X_1-\frac{1}{K}]\leq 0}}}
% $$
\subsubsection{A simple case: $\Exp{X_1}=1/K$.}
\textcolor{red}{Need to check that didn't reach a minimizer of expected payoff somehow}
Here we consider that $X_1$ is GP($\sigma_1,\xi_1$), with 
$$
\frac{\sigma_1}{1-\xi_1}=\frac{1}{K}\;.
$$

\begin{lemma}\label{lemma:shadingForGPsAgainstUnifAdversariesSimple}
In this setup, when player 1 faces $K$ adversary with Unif$[0,1]$ values who play truthfully, the optimal solution is to shade through 
$$
X_t=\frac{1}{1-\xi_1} \frac{K}{K+1}X_1\;.
$$
\end{lemma}

\textbf{Application}: assume we have 3 players with Unif$[0,1]$ values, only one of each is strategic. Then the strategic player needs to shade her bid through 
$$
X_t=\frac{1}{2}\beta^{I}(X_1)\;,
$$ 
where $\beta^{I}(X_1)$ is her first price bid. This is immediate since Unif$[0,1]$ are GP($1,-1$). 

\begin{proof}[Proof of Lemma \ref{lemma:shadingForGPsAgainstUnifAdversariesSimple}]
In this case, $\Exp{X_1}=\frac{1}{K}$, so there is a chance that 
$K/(K+1) (X_1-1/K)$ be a virtual value, since that random variable has mean 0. 

We note that if $Y$ is GP($\sigma,\xi$), $\alpha Y$ is GP($\sigma \alpha,\xi$). 

Let us consider 
$$
X_t=\frac{1}{1-\xi_1}\frac{K}{K+1} X_1\;.
$$
If $X_1$ is GP($\sigma_1,\xi_1$), $X_t$ is GP($\frac{\sigma_1}{1-\xi_1}\frac{K}{K+1}\sigma_1,\xi_1$). In particular, calling $(\sigma_t,\xi_t)$ the GP parameters of $X_t$, we have 
$$
\frac{\sigma_t}{1-\xi_t}=\frac{\sigma_t}{1-\xi_1}=\frac{\sigma_1}{1-\xi_1}\frac{K}{K+1}\sigma_1=\frac{1}{K+1}\;,
$$
since $\sigma_1/(1-\xi_1)=1/K$. 
We conclude that 
\begin{align*}
\phi_t(X_t)&=(1-\xi_1) X_t-\frac{\sigma_t}{1-\xi_t}=(1-\xi_1) X_t-\frac{1}{K+1}\\
&=\frac{1-\xi_1}{1-\xi_1}\frac{K}{K+1} X_1-\frac{1}{K+1}\\
&=\frac{K}{K+1}\left(X_1-\frac{1}{K}\right)=\frac{1}{1+\frac{1}{K}}(X_1-\frac{1}{K})\;.
\end{align*}
We conclude that $\phi_t(X_t)$ has the desired form. 
\end{proof}
\subsection{Other GPs}
In general for GPs, we have 
$$
\frac{F_W}{f_W}=\sigma (1+\frac{\xi t}{\sigma})^{1+1/\xi}-\xi t-\sigma\;.
$$
Since $c_\phi=(1-\xi)$ and $c_\phi r^*=\sigma$, we get that 
$$
\frac{F_Z}{f_Z}=c_\phi\frac{F_W(\phi^{-1}(t))}{f_W(\phi^{-1}(t))}=
\sigma (1-\xi) (1+\frac{(t+\sigma)\xi }{\sigma (1-\xi)})^{1+1/\xi}-\xi t-\sigma\;.
$$
So we get that 
\begin{align*}
t+\frac{F_Z}{K f_Z}(t)&=(1-\frac{\xi}{K}) t+\frac{\sigma(1-\xi)}{K}\left[1+\xi \frac{t+\sigma}{\sigma (1-\xi)}\right]^{1+1/\xi}-\frac{\sigma}{K}\;,\\
&=(1-\frac{\xi}{K}) t + \frac{\sigma(1-\xi)^{-1/\xi}}{K}\left[1+\frac{\xi t}{\sigma}\right]^{1+1/\xi}-\frac{\sigma}{K}\;.
\end{align*}
For uniform, $\xi=-1$, $\sigma=1$ so we recover the above result. 


\subsection{Miscellaneous computations}
\subsubsection{A key relation}

Let $X$ be a non-negative r.v and $\phi$ be its virtual value function, which is assumed to be increasing. 

Let $t \in \mathbb{R}$. Then 
\begin{align*}
\Exp{\phi(X)1_{X\leq t}}&=\int_0^t (x-\frac{1-F(x)}{f(x)}) f(x) dx\;,\\
&=\int_0^t xf(x) dx -t +\int_0^t F(x) dx\;,\\
&=\left. xF(x)\right|_0^t -\int_0^t F(x) dx -t +\int_0^t F(x) dx\;,\\
&= t \left[F(t)-1\right]\;.
\end{align*}
In particular, 
\begin{align*}
\Exp{\phi(X)1_{\phi(X)\leq t}}&=\Exp{\phi(X)1_{X\leq \phi^{-1}(t)}}\;,\\
&=\phi^{-1}(t) \left[F(\phi^{-1}(t))-1\right]\;,\\
&=\phi^{-1}(t) \left[P(X\leq \phi^{-1}(t))-1\right]\;,\\
&=\phi^{-1}(t) \left[P(\phi(X)\leq t)-1\right]\;,\\
&=- \phi^{-1}(t) P(\phi(X)> t)\;.
\end{align*}
We conclude that 
$$
\phi^{-1}(t)=\frac{\Exp{\phi(X)1_{\phi(X)\leq t}}}{P(\phi(X)\leq t)-1}\;.
$$
\subsubsection{Another important relation}
\textcolor{red}{This is also what we have at the very beginning of the note...}
\begin{lemma}
Suppose $X_t=g(X_1)$, where $g$ is invertible. If $x_t=g(x_1)$, we have 
$$
\phi_t(x_t)=g(x_1)+g'(x_1)[\phi_1(x_1)-x_1].
$$
\end{lemma}
In particular, it is very easy to find a random variable such that $\phi_t(X_t)$ has a given form (as a function of $X_1$) on an interval... Note also $[\phi_1(x_1)-x_1]$ is just one over the hazard rate of $X_1$ evaluated at $x_1$. 

\begin{proof}
If $X_t=g(X_1)$, $F_t(x)=P(X_t\leq x)=P(g(X_1)\leq x)=F_1(g^{-1}(x))$. Hence, 
$$
f_t(x)=f_1(g^{-1}(x))\frac{1}{g'(g^{-1}(x))}\;.
$$
Therefore, 
\begin{align*}
\phi_t(x)&=x-\frac{1-F_t(x)}{f_t(x)}\\
&=x-g'(g^{-1}(x))\frac{1-F_1(g^{-1}(x)}{f_1(g^{-1}(x))}\\
&=x+g'(g^{-1}(x))\left[\phi_1(g^{-1}(x))-g^{-1}(x)\right]\;.
\end{align*}
Therefore, 
$$
\phi_t(x_t)=\phi_t(g(x_1))=g(x_1)+g'(x_1)\left[\phi_1(x_1)-x_1\right]
$$
\end{proof}

\subsubsection{A key ODE}
Venturing further, it seems that if we write $X_t=g(X_1)$, the key equation to solve is 
$$
\phi_t(X_t)=(\id + \frac{F}{f})^{-1} X_1\;, \phi_t(X_t)\geq 0\;. 
$$
Calling $h=(\id + \frac{F}{f})^{-1}$, the question becomes: can we solve 
$$
\phi_t(x_t)=\phi_t(g(x_1))=g(x_1)+g'(x_1)\left[\phi_1(x_1)-x_1\right]=h(x_1)\;.
$$
This looks simple enough: elementary manipulations point to taking 
$$
g(x)=\frac{g(x_0)(1-F_1(x_0))-\int_{x_0}^x h(u) f_1(u) du}{1-F_1(x)}\;.
$$
Indeed, 
$$
\phi_t(x_t)=g(x_1)-\frac{1-F_1(x_1)}{f(x_1)}g'(x_1)=\frac{1}{f(x_1)} (g(x_1)(F_1(x_1)-1))'\;.
$$
Now one needs to check that inverting $\id+F/f$ is possible and/or necessary. Also we need to satisfy the equation only for $\phi_t(x_t)\geq 0$, which gives a condition on $g$/$x_0$. Also, obviously, is $g$ non-negative... Take $x_0=+\infty$  and be done with problems?

We note further the elementary fact that for an invertible function $\gamma$, 
$$
\int_{\alpha}^\beta \gamma^{-1}(u)f_1(u) du = 
\int_{\gamma^{-1}(\alpha)}^{\gamma^{-1}(\beta)} t f_1(\gamma(t)) \gamma'(t) dt\;,
$$
so the computation of $g$ may not be too hard if all the above makes sense. 
\textcolor{red}{requiring $\id+F/f$ to be invertible is a bit overkill. It should just be surjective/onto I think. Having an ansatz for $\phi_t(x_t)$ should be enough and then re-inject in equation.}
\subsubsection{Equilibrium question?}
So recall that if we shade to send $x_t=g(x)$, $\phi_t(x_t)=g(x)-xg'(x)+g'(x) \phi_X(x)$. Let's call this $h(x)=\phi_t(x_t)$. 
So if we are in a symmetric equilibrium, everybody will use this shading. Recall that the key relation was 
$$
(x_1-\phi_t(x_t))f_Z(\phi_t(x_t))-F_Z(\phi_t(x_t))=0\;, \text{ for } \phi_t(x_t)\geq 0\;.
$$
Let's see if we can get an ODE out of this. $Z$ is the random variable representing the max of the virtual values of the competition and 0. So for positive argument it's a standard max. In particular, if $F_t$ is the cdf of $\phi_t(X_t)$, $F_Z(t)=F_t^{K-1}(t)$ for positive $t$'s. 

If $W=h(X)$, 
$$
F_W(t)=P(W\leq t)=P(h(X)\leq t)=P(X\leq h^{-1}(t))=F_X(h^{-1}(t))\;.
$$
So 
\begin{align*}
F_W(t)&=F_X(h^{-1}(t))\;, &f_W(t)&=\frac{1}{h'(h^{-1}(t))} f_X(h^{-1}(t))\;,\\
F_W(h(x))&=F_X(x)\;, &f_W(h(x))&=\frac{f_X(x)}{h'(x)}\;.
\end{align*}
So if we face $K-1$ adversaries, it seems that at equilibrium we would have 
$$
(x-h(x))(K-1)\frac{f_X(x)}{h'(x)}=F_X(x)\;,
$$
or 
\begin{gather}\label{eq:EquilibriumShadingTentative}
\boxed{(K-1)(x-h(x)) f_X(x)-h'(x)F_X(x)=0}\;, h(x)\geq 0\\
h(x)=g(x)-xg'(x)+g'(x) \phi_X(x)\;. \notag
\end{gather}
Because $h(x)=g(x)-xg'(x)+g'(x) \phi_X(x)$ this is a second degree equation in the shading function $g$. Note however that if the computations in the previous subsections are correct, we know how to compute $g$ from $h$. 

We note that the solution of Equation \eqref{eq:EquilibriumShadingTentative} (\textcolor{blue}{very much first price}...) is 
$$
\text{if } h=C h_0 F^{-(K-1)}, h_0'=\frac{K-1}{C}xf_X(x) F^{K-2}
$$
So one solution is
$$
h(x)=\frac{\int_0^x yg(y) dy}{G(x)}\;, \text{ where } G(x)=F^{K-1}(x)\;.
$$
So $h(x)=\Exp{Y_1|Y_1<x}$, where $Y_1$ is the maximum bid of our $K-1$ adversaries. This of course is nothing but a first price bid, see \cite{krishna2009auction}, p. 15. 

\textcolor{blue}{Interpretation??: do we shade so that we end up paying first price in virtual value space?} And then we just need to solve the ODE that corresponds to first price shading... And that should be easy, if nothing goes awry, since we have a closed form expression for $g$ as a function of $h$. 
\begin{lemma}[\textcolor{red}{Still a bit tentative and to be double checked but should be right}]
In the symmetric case and for the Myerson auction, an equilibrium strategy for the bidders is to shade their bids by a function $g$ that satisfies 
$$
g(x)+g'(x)(\phi_X(x)-x)=\beta^{I}(x)\;,
$$
where $\beta^{I}(x)$ is their first price bid. 

A solution of this equation is 
$$
g(x)=\Exp{\beta^{I}(X)|X\geq x}\;,
$$
leading to the shading 
$$
X_t=g(X_1)=\Exp{\beta^{I}(X)|X\geq X_1}\;.
$$
With this strategy, their expected payoff is the same as what they would get in a first price auction. 
\end{lemma}
\textcolor{red}{Triple check that this is indeed the solution we want; proof below is for it though.}
\begin{proof}
Aggregate all the results above and make sure everything sticks.
Note that there is easy conditional expectation interpretation... 

We note that $\beta^{I}(x)$ is an increasing function of $x$. Furthermore, if $g$ is a solution of 
$$
g(x)+g'(x)(\phi_X(x)-x)=h(x)\;,
$$
such that 
$$
g(x)=\frac{\int_x^{\infty}h(u)f(u) du}{1-F(x)}\;,
$$
we have, if we re-interpret this equation, 
$$
g(x)=\Exp{h(X)|X\geq x}\;.
$$
Now consider $F_{t_1}$ (resp. $F_{t_2}$) the cdf of $X|X\geq t_1$. If $t_1\geq t_2$, it is easy to see that the ratio 
$$
\frac{f_{t_1}(x)}{f_{t_2}(x)} \text{ is non-decreasing}. 
$$
Therefore, the distribution $F_{t_1}$ dominates $F_{t_2}$ in terms of likelihood ratio (see \cite{krishna2009auction}, Appendix B, p. 276). In particular, this implies that the function $g$ is non-decreasing (since likelihood ratio dominance implies first order stochastic dominance). In our case, simple modifications of the arguments given in Appendix B of \cite{krishna2009auction} can be used to show that $g$ is actually increasing. 

We conclude that our function $g$ is invertible. It is then trivial to verify the differential equation aspects of the proof. 

Almost by definition, we have 
$$
\phi_t(x_t)=\beta^{I}(x_1)=\beta^{I}(g^{-1}(x_t))\;.
$$
Since $g$ is increasing, so is $g^{-1}$; and since $\beta^{I}$ is increasing, so is $\beta^{I}(g^{-1}(x))$. We conclude that $\phi_t$ is increasing and so the design problem for the seller receiving $X_t$ is regular. (In particular, no ironing will be needed to perform the Myerson auction; in particular, the problem we solved is exactly the one faced by the seller\footnote{if $\phi_t$ had not been regular, then the Myerson auction would have involved not $\phi_t$ but an ironed out version of this function; optimizing this would have been horrible}.)

Now as we are in the symmetric case, if our adversaries use this strategy, our opposition in virtual value space is $Z=\max(0,\phi_i(g_i(X_i)))=\max(0,\beta^{I}(X_i))=\max(\beta^{I}(X_i))$. 
So the distribution of $Z$ is continuous, it has no discontinuity at 0. 
In particular, for the functional derivative of our payoff we have 
$$
\frac{\partial}{\partial t} \Pi(t)=\Exp{\frac{\partial}{\partial t} \phi_t(X_t) [(X_1-\phi_t(X_t))f_Z(\phi_t(X_t)-F_Z(\phi_t(X_t)]}\;.
$$
Now we have done everything so that 
$$
[(x_1-\phi_t(x_t))f_Z(\phi_t(x_t)-F_Z(\phi_t(x_t)]=0
$$
everywhere. 

\textcolor{red}{we used the ansatz strongly to get rid of the troublesome max(0,something). So it's really a verification proof. We're lucky because the easy case seems to work.}

\textcolor{red}{still need to check that the constants make sense etc...}
\end{proof}

\paragraph{Conclusion} if previous thing is true: no need to organize complicated auctions. Strategic buyers will be able to get expected payoff of first price auction. 

\paragraph{Interpretation}: from the buyer's standpoint, the payoff of the Myerson auction corresponds in expectation to a ``first  price auction in virtual-value-bid space". It is then natural for the buyer to seek to bid as in a first price auction. Naturally, she needs to ensure that after her bid is transformed into a virtual value bid, she indeed pays a standard first price. The first order differential operator that plays a key role in the Myerson auction renders this constraint easy to satisfy. 
\paragraph{Miscellaneous: } why is it not a minimum of revenue? We show by econ arguments that the buyer expected payoff is higher than with no shading. Note that the payoff of the buyer is that of a first price auction with no reserve price. By revenue equivalence, this is the same as her payoff in a second price auction with no reserve price. However the Myerson auction in the case of symmetric buyers is a second price auction with reserve price as the monopoly price. Hence the buyer's payment is higher with no shading than with the shading we propose. 

\subsubsection{General comment}
In some sense we managed to solve the problem because we could write in a sufficiently nice way the payoff function as a function of our shading function $g$
$$
\Pi(t)=\Exp{L(X_1,X_t=g(X_1),F_Z,g)}\;, where 
$$
$X_1$ is our value, $g(X_1)$ is the shaded value we send, $F_Z$ is the distribution of ``the bids" of the adversaries. Taking a differential in function space led to a differential equation for $g$ involving the distribution of $X_1$, and $F_Z$ (and functions of it). 
We should be able to follow a similar strategy for other types of auctions than the Myerson auction... For instance second price auctions with reserve price set at the monopoly price, see above. (Note that off symmetry it's not the same as Myerson, so as we need to get off symmetry to find the equilibrium strategy it's not obvious a priori that shading strategy will be same as above). 

For the second price auction with monopoly reserve price, if we denote by $B$ the bids of the adversaries (note that depending on the particular rules of that auction (lazy or not) the distribution of $Z$ will vary), if shading by $X_t$ we will win only when $X_t\geq Z=\max(B,\phi_t^{-1}(0))$, in which case we will pay $Z$. 
So the expected payoff is of the form 
$$
\Pi(t)=\Exp{(X_1-Z)1_{X_t\geq Z}}\;.
$$
Using independence of $Z$ and $X_t$ we get after computations (that have not been carefully verified), if $T_g\triangleq \phi^{-1}_t(0)$, 
\begin{align*}
\Pi(t)&=\Exp{X_1 F_B(X_t) 1_{X_t\geq T_g }}\\
&-\Exp{X_1\left[X_t F_B(X_t)-\int_{T_g}^{X_t} F_B(u) du \right]1_{X_t\geq T_g}}\;.
\end{align*}
When $\phi_t$ is increasing, i.e. when $X_t$ has a regular distribution, $X_t\geq T_g$ is equivalent to $\phi_t(X_t)\geq 0$, so the previous equation becomes 
\begin{align*}
\Pi(t)&=\Exp{X_1 F_B(X_t) 1_{\phi_t(X_t)\geq 0 }}\\
&-\Exp{X_1\left[X_t F_B(X_t)-\int_{T_g}^{X_t} F_B(u) du \right]1_{\phi_t(X_t)\geq 0}}\;.
\end{align*}

\subsubsection{Boosted second price auctions}
Make sure that in a general sense the payoff for the buyer is of the form $\Exp{[X_1-\gamma_t(X_t)]F_Z(\gamma_t(X_t))}$. Then as function of operator $\gamma_t$ find a good shading strategy. 

If can write boosted 2nd price like that, i.e. just say that regardless of adversary we end having a Myerson-like payoff, with $Z$ depending on boosting, then the problem is a ``simple" 2-parameter optimization problem.  

Would be interesting in general to write it as a functional optimization with equality constraints involving a nice differential operator. 

Outside of the uniform adversaries above probably don't end up with with a mapping from GPs to things that are pretty much GPs. 

\subsubsection{An integral involving GPs}
Suppose $F_1(x)=1-(1+\xi x/\sigma)^{-1/\xi}$, i.e $X$ is $GP(\sigma,\xi)$. For its density we have $f_1(x)=\frac{1}{\sigma}(1+\xi x/\sigma)^{-1/\xi-1}$ on $[0,-\sigma/\xi]$. 
A tedious computation shows that 
$$
\int_x^{-\sigma/\xi} u f_1(u) du =\frac{\sigma}{\xi}\left[\frac{1}{1-\xi}\left(1+\frac{\xi x}{\sigma}\right)-1\right](1-F_1(x))\;.
$$
The conclusion is that 
\begin{equation}\label{eq:meanGPs}
r(x)=\frac{\int_x^{-\sigma/\xi} u f_1(u) du }{1-F_1(x)}=\frac{x+\sigma}{1-\xi}\;.
\end{equation}
Note that, as is obvious from the integral definition,  $$
r(x)\geq x\;,
$$
because 
$$
r(x)=\frac{x+\sigma}{1-\xi}=x+\frac{\sigma}{1-\xi}(1+\xi x/\sigma)\geq x\;, \text{ since } x\leq -\frac{\xi}{\sigma}\;. 
$$



==> pWinIncrease.tex <==
\section{How to increase our Pwin only}
%this is a set of differential computations for moving infinitesimally reserve price etc...
%the take-away message of this is that the "right control" or a good way to do stuff is to work on the hazard rate directly... may not make it to final version of paper.


In these short notes, we explain how to increase against the reserve price by doing modelization in the hazard rate space. 
We also explain to what non-linear shading that corresponding in the bid world. 
This is extremely rough and will need to be verified. 

The main idea is to do differential computations in hazard rate space, as a way of getting a PDE (or a system of PDEs) for how the bidders should play. So the $\eps$ below should be thought of as dt fundamentally...


We call $\lambda$ the hazard rate of the random variable $X$. We assume that $X\geq 0$ because it corresponds to our setting.  For simplicity for below, we assume that $\lambda$ is continuous, $\lambda(0)=0$ and to temporarily avoid thinking about distributions whose support is a subset of $\mathbb{R}^+$, we assume that $\lambda(x)>0$ on $\mathbb{R}^+$. We also consider regular distributions in the sense of Myerson, so $x-1/\lambda(x)$ is an increasing function of $x$. Implicitly we assume below that the perturbation leave the perturbed distribution regular, so that the reserve price is indeed set at $\vValue^{-1}(0)$ Note that in hazard rate terms Myerson's requirement for the monotonicity of the virtual value function means that  
\begin{equation}
1+\lambda'/\lambda^2>0 \;. \tag{Myerson-Monotonicity}
\end{equation}
As we will sometime use the hypothesis that $\lambda_0=0$, this will force us to consider perturbations $\eta$'s such that $\eta'(0)=0$, which is not a big requirement. 
\subsection{Reserve price manipulation}

Recall that
$$
1-F(x)=\exp(-\int_0^x \lambda(u) du)\;.
$$
Call $\lambda_\eta=\lambda+\epsilon \eta$. The probability of clearing the reserve price with $X$ is just on a log-scale, 
$$
 \log P(X\geq \vValue^{-1}(0))= \log(1-F(\vValue^{-1}(0)))=-\int_0^{\vValue^{-1}(0)} \lambda (t) dt\;.
$$
Note that if $x_0=\vValue^{-1}(0)$, $x_0=1/\lambda(x_0)$. Let us now call $x_\eta=\vValue_{\lambda+\eta \epsilon}^{-1}(0)=x_0+\delta$. Then 
\begin{align*}
x_0+\delta &=\frac{1}{\lambda(x_0+\delta)+\epsilon \eta(x_0+\delta)}\;,\\
&\simeq \frac{1}{\lambda(x_0)+\lambda'(x_0) \delta +\epsilon\eta(x_0)}\;,\\
&=\frac{1}{\lambda(x_0)}\left(1-\frac{\delta \lambda'(x_0)+\epsilon \eta(x_0)}{\lambda(x_0)}\right)\;,\\
&=x_0-x_0^2(\delta \lambda'(x_0)+\eps \eta(x_0))\;.
\end{align*}

Hence, 
\begin{equation}
\boxed{
\delta=-\epsilon \frac{\eta(x_0)x_0^2}{1+x_0^2\lambda'(x_0)}=-\eps \frac{\eta(x_0)}{\lambda^2(x_0)+\lambda'(x_0)}\;.}\tag{resPrice-Pertub}
\end{equation}
\textbf{Interpretation} This formula has a nice and simple interpretation. Indeed, since $x_0^2=1/\lambda(x_0)^2$, the numerator is just $\vValue'(x_0)$, which is not surprising. In particular, if $\vValue$ is borderline regular near $x_0$, a small pointwise modification of $\lambda$ will result in an important change in reserve price. Note that by picking $\eta$ such that $\eta(x_0)$ is pointwise very large but $\int \eta(t)$ is very small we do very little to perturb the cdf but impact  the reserve price. A natural idea is to pick $\eta(t)$ to have a graph like a hugely elongated triangle. The area of the triangle may be super small while $\max_t(\eta(t))$ is huge. One thing to consider nonetheless is that if we want to maintain regularity, we need 
$$
1+\frac{\lambda'+\eps \eta'}{(\lambda+\eps \eta)^2}>0\;,
$$
with $\eta'$ being potentially a subgradient. So the steepness of $\eta$ would have to be controlled by the value of $\lambda'$

\subsection{Probability of exceeding the reserve price}

We conclude that with $x_0=\vValue^{-1}(0)$, using continuity of $\lambda$ at $x_0$ and $x_0=1/\lambda(x_0)$, 
$$
\boxed{
\log[P_\eta(X_\eta\geq \phi_\eta^{-1}(0)]\simeq \log(P(X\geq \vValue^{-1}(0)))-\epsilon \left[\int_0^{x_0} \eta(t) dt -\frac{\eta(x_0)x_0}{1+x_0^2\lambda'(x_0)}\right]\;.
}
$$
\subsection{How to implement a (perturbative) non-linear shading}
On the other hand, if $Y=\beta(X)$, with $\beta$ one-to-one and $\gamma=\beta^{-1}$, we see that 
$$
\forall t\;, \int_0^t \lambda_Y(t) dt= \int_0^{\gamma(t)} \lambda_X(t) dt\;.
$$
Let's assume that $\lambda_Y(t)=\lambda_X(t)+\epsilon \eta(t)$; we now seek $\gamma$ of the form $\gamma(x)=x+\epsilon \nu(x)$.

After differentiation and re-arrangement, we get that 
$$
\eta(t)=(\nu(t)\lambda(t))'\;.
$$
Hence, 
$$
\nu(t)\lambda(t)-\nu(0)\lambda(0)=\int_0^x \eta(u) du\;.
$$
On the other hand, we have $\beta(x)\simeq x-\epsilon \nu(x)$ and hence
$$
\beta(x)=x-\epsilon\nu(x)\;.
$$
So roughly speaking, 
$$
\beta(x)=x-\epsilon\nu(x)=x-\epsilon \frac{\nu(0)\lambda(0)+\int_0^x \eta(u) du}{\lambda(x)}\;.
$$
Focusing, on the case where $\lambda(0)=0$, which roughly speaking means that $f(0)=0$, a reasonable situation for us, then we have 
\begin{equation}
\beta(x)=x-\epsilon \frac{\int_0^x \eta(t) dt}{\lambda(x)}\;. \tag{non-lin-Shading}
\end{equation}
In particular, if $\eta$ is picked to solve an optimization problem such as lowering reserve price under revenue constraint, we can then shade our bids accordingly by using the above formula. 


\textcolor{red}{All that is below is tentative; comps need to be redone and verified. aim: formulate optim problem for non-linear shading}
\subsection{Impact of perturbation on payoff}
\subsubsection{Beating another random variable}
The motivation here is second price auctions with individual reserve prices. 

Another potentially useful result is that if $Y$ is a random variable independent of $X$, we have, if $g$ is the density of $Y$, 
$$
P_{\eta}(X_\eta\geq Y)\simeq P_0(X_0\geq Y)-\epsilon \int \eta(t) dt \int_t^{\infty} g(y) P(X_0\geq y) dy\;.
$$
We can rewrite $\int_t^{\infty} g(y) P(X_0\geq y) dy=P(t\leq Y\leq X_0)$, so that 
$$
P_{\eta}(X_\eta\geq Y)\simeq P_0(X_0\geq Y)-\epsilon <\eta(t),P(t\leq Y\leq X_0)>\;.
$$
From this we conclude about the impact of a perturbation of $\lambda$ on our PWin. 
Indeed, in the second price setting with individual reserve prices, if $Y$ denotes the largest value for the opponents having beaten their reserve price, for the overall $PWin$, 
$$
PWin=P(X\geq \max(\vValue^{-1}(0),Y))\;.
$$

Another way to re-write this is that, to first order, 
\begin{align*}
PWin_\eta&=\int_{x_0+\delta}^\infty P(X_\eta\geq y) g(y) dy\\
&= \int_{x_0}^\infty P(X_0\geq y) \me^{-\eps \int_0^y \eta(t) dt }g(y) dy +\delta P(X_0\geq x_0) \me^{-\eps \int_0^{x_0} \eta(t) dt} g(x_0)\\
&= Pwin_0 -\eps \int \eta(t) P(\max(t,x_0)\leq Y\leq X_0) dt \\
&+\delta P(X_0\geq x_0)  g(x_0)
\end{align*}
So 
\begin{gather*}
PWin_\eta-PWin_0\\
=\\
-\eps \int \eta(t) P(\max(t,x_0)\leq Y\leq X_0) dt -\eps \frac{\eta(x_0)g(x_0)}{\lambda^2(x_0)+\lambda'(x_0)}(1-F(x_0))
\end{gather*}

Based on data we (potentially) have access for $t\geq x_0$ to estimates of $P(X_0\geq Y\geq t)$ by looking at costs of 2nd price auctions with reserves. Otherwise, all we know is that this quantity is between 0 and 1. 

A similar computation can be made for expected payoff. 
\\

\subsubsection{Myerson}

Indeed, for the $PWin$ computation, we require 
$$
P_\eta(\vValue_\eta(X_\eta)\geq Y)=\int [f_\eta(x) P(\vValue(x)\geq Y)+\eps \frac{\eta f_\eta}{\lambda^2}g(x)]dx\;.
$$

Using computations below, we get that 
\begin{align*}
&P_\eta(\vValue_\eta(X_\eta)\geq Y)=P(\vValue(X)\geq Y)\\
&+ \eps \int \frac{\eta}{\lambda^2} g(x) f(x) dx +\eps \int dx
P(\vValue(x)\geq Y)(\eta (1-F_0)-\int_0^x \eta(t) dt)
\end{align*}

\subsubsection{A look at expected reward}
Now, we also have $\vValue_\eta(x)\simeq \vValue(x)+\eps \eta/\lambda^2.$
We assume that for all practical purposes we can linearize 
$$
\exp(-\eps \int_0^x \eta(t) dt)\simeq 1-\eps \int_0^x \eta(t) dt\;.
$$
For large $x$ that is potentially problematic, but our approximations are easy to make rigorous if the above approximation is valid where most of the action in the integral is going on. 
We note that 
\begin{align*}
f_\eta(x)&=\lambda_\eta (1-F_0) \exp(-\eps \int_0^x \eta(t) dt)=[f_0+\eps \eta (1-F_0)] \exp(-\eps \int_0^x \eta(t) dt)\;,\\
P_\eta(x\geq y)&=(1-F_0(y)) \exp(-\eps \int_0^y \eta(t) dt)\;,\\
P_Y(\vValue_\eta(x)\geq Y)&=P_Y(\vValue(x)\geq Y)+\eps \frac{\eta(x)}{\lambda^2(x)}g(x)\;.
\end{align*}
Hence, the bidder's expected payoff can be written as 
\begin{align*}
\Pi_\eta&=\int_{\mathbf{x_0+\delta}}^\infty (\lambda-\eps \frac{\eta}{\lambda^2})f_\eta(x)[P_Y(\vValue(x)\geq Y)+\eps \frac{\eta}{\lambda^2} g(x)]dx\;,\\
&= \int_{\mathbf{x_0}}^\infty (\lambda-\eps \frac{\eta}{\lambda^2})f_\eta(x)[P_Y(\vValue(x)\geq Y)+\eps \frac{\eta}{\lambda^2} g(x)]dx\\
&+\delta \lambda(x_0) f(x_0) P_Y(0\geq Y)\;,
\end{align*}
where 
$$
\lambda(x_0)=1/x_0 \text{ and } \delta=-\epsilon \frac{\eta(x_0)x_0^2}{1+x_0^2\lambda'(x_0)}\;.
$$

After expanding the quantity under the integral we find that it is equal to
\begin{gather*}
\lambda(x) P_Y(\vValue(x)\geq Y) f_0(x)\\
+\\
\eps\left\{ P_Y(\vValue(x)\geq Y)[\eta f_0-\frac{f_0^2}{1-F_0}\int_0^x \eta(t) dt-\frac{f_0\eta}{\lambda^2}]+\frac{\eta}{1-F_0}g\right\}
\end{gather*}
We note that $f_0/\lambda^2=(1-F_0)^2/f_0^2\;.$

After regrouping the terms, we find that 
$$
\Pi_\eta=\Pi_0+\eps \left[\int_{0}^{\infty}\eta(t) \Gamma_0(t) dt -\frac{\eta(x_0)x_0 f(x_0)}{1+x_0^2 \lambda'(x_0)}\right]\;.
$$

Note that to compute $\Gamma_0$, we just need to know $f_0$, $1-F_0$, $g$ and $\int_x^\infty f_0^2(u)/(1-F_0(u))[u\geq x_0] du$.
